Object-oriented Programming Laws for Annotated Java Programs

Object-oriented programming laws have been proposed in the context of languages that are not combined with a behavioral interface specification language (BISL). The strong dependence between source-code and interface specifications may cause a number of difficulties when transforming programs. In this paper we introduce a set of programming laws for object-oriented languages like Java combined with the Java Modeling Language (JML). The set of laws deals with object-oriented features taking into account their specifications. Some laws deal only with features of the specification language. These laws constitute a set of small transformations for the development of more elaborate ones like refactorings.

==> eptcsdata.tex <==
\providecommand{\event}{I. Mackie and A. Martins Moreira (Eds.): Tenth International\\Workshop on Rule-Based Programming (RULE 2009)}
\providecommand{\volume}{21}
\providecommand{\anno}{2010}
\providecommand{\firstpage}{65}
\providecommand{\eid}{6}

